The Power of Exploiter: Provable Multi-Agent RL in Large State Spaces

Modern reinforcement learning (RL) commonly engages practical problems with large state spaces, where function approximation must be deployed to approximate either the value function or the policy. While recent progresses in RL theory address a rich set of RL problems with general function approximation, such successes are mostly restricted to the single-agent setting. It remains elusive how to extend these results to multi-agent RL, especially due to the new challenges arising from its game-theoretical nature. This paper considers two-player zero-sum Markov Games (MGs). We propose a new algorithm that can provably find the Nash equilibrium policy using a polynomial number of samples, for any MG with low multi-agent Bellman-Eluder dimension -- a new complexity measure adapted from its single-agent version (Jin et al., 2021). A key component of our new algorithm is the exploiter, which facilitates the learning of the main player by deliberately exploiting her weakness. Our theoretical framework is generic, which applies to a wide range of models including but not limited to tabular MGs, MGs with linear or kernel function approximation, and MGs with rich observations.

==> OLIVE_MG.tex <==
\pagebreak
\section{\olive\ for Markov Games}
\subsection{algorithm}

\begin{algorithm}[h]
    \caption{\olivemg\ $(\Fcal,\Gcal,K,\nactout,\nelimout,\zetaactout,\zetaelimout,\nactin,\nelimin,\zetaactin,\zetaelimin$) }
    \label{alg:olivemg}
    \begin{algorithmic}[1]
     \STATE \textbf{Initialize}:  $\Dcal_1,\dots,\Dcal_H\leftarrow \emptyset$, $\Bcal^0 \leftarrow \Fcal$.
     \FOR{\textbf{episode} $k$ from $1$ to $\kout$} 
     \STATE \textbf{Choose policy} $\mu^k = \mu_{f^k}$, where $f^k = \argmax_{f \in \Bcal^{k-1}}\nash(f_1,s_1)$. 
    \STATE \textbf{Compute} $\nu^k=$\olivebr$(\Gcal,\mu^k,\kin,\nactin,\nelimin,\zetaactin,\zetaelimin)$.
    \STATE \textbf{Refresh} $\Dcal$ and sample $\nactout$ trajectories by following $\pi^k:= (\mu^k,\nu^k)$.
    \STATE \textbf{Estimate} $\hatberr{ f^k, \pi^k, h}$ for all $h\in[H]$, where 
    \begin{align*}
    \hatberr{f, \pi^k, h} = \frac{1}{|\Dcal_h|} \sum_{(s,a,b,r,s') \in \Dcal_h}\left(f_h(s,a,b)-r - \max_{a'\in\Acal}\min_{b'\in\Bcal} f_{h+1}(s',a',b')\right).
    \end{align*} 
    \IF{$\sum_{h=1}^H \hatberr{f^k, \pi^k,h} \le H\zetaactout$}
    \STATE \textbf{Terminate} and output $\mu^k$.
    \ELSE
    \STATE \textbf{Execute} $\pi^k$ for $\nelimout$ episodes and \emph{refresh} $\Dcal_h$ to include the fresh $(s_h,a_h,r_h,s_{h+1})$ tuples.
    \vspace{-4mm}
    \STATE \textbf{Estimate}  $\hatberr{f, \pi^k, t}$ for all $f\in \Bcal^{k-1}$ and Update
    $$\Bcal^{k} = \left\{f \in \Bcal^{k-1} : \left|\hatberr{f,\pi^k,t} \right|\le \zetaelimout \right\}.$$
    \ENDIF
    \ENDFOR
    \end{algorithmic}	
    \end{algorithm}
    
    \tiancheng{reset counter}

    \setcounter{algorithm}{0}
    \begin{routine}[h]
    \caption{\olivebr$(\Gcal,\mu,\kin,\nactin,\nelimin,\zetaactin,\zetaelimin)$}
    \label{alg:olivemg-routine}
    \begin{algorithmic}[1]
    \STATE \textbf{Initialize}:  $\Dcal_1,\dots,\Dcal_H\leftarrow \emptyset$, $\Ccal^0 \leftarrow \Gcal$.
    \FOR{\textbf{episode} $k$ from $1$ to $\kin$}
    \STATE \textbf{Compute} $g^k = \argmin_{g\in\Ccal^k} \min_{b}{\mu^k_{1}(s_1)}\trans g_{1}(s_1,\cdot,b)$ and let $\nu^k$ be the greedy policy w.r.t. ${\mu^k}\trans g^k$.
    \STATE \textbf{Refresh} $\Dcal$ and sample $\nactin$ trajectories by following $\pi^k:= (\mu^k,\nu^k)$.
    \STATE \textbf{Estimate} $\hatberr{ g^k, \pi^k, h}$ for all $h\in[H]$, where 
    \begin{align*}
    \hatberr{g, \pi^k, h} = \frac{1}{|\Dcal_h|} \sum_{(s,a,b,r,s') \in \Dcal_h}\left(g_h(s,a,b)-r - \min_{b'\in\Bcal}{\mu^k}\trans g_{h+1}(s',b')\right).
    \end{align*} 
    \IF{$\sum_{h=1}^H \hatberr{g^k, \pi^k,h} \le H\zetaactin$}
    \STATE \textbf{Terminate} and output $\nu^k$.
    \ELSE
    \STATE \textbf{Execute} $\pi^k$ for $\nelimin$ episodes and \emph{refresh} $\Dcal_h$ to include the fresh $(s_h,a_h,r_h,s_{h+1})$ tuples.
    \vspace{-4mm}
    \STATE \textbf{Estimate}  $\hatberr{g, \pi^k, t}$ for all $g\in\Ccal^{k-1}$ and Update
    $$\Ccal^{k} = \left\{g \in \Ccal^{k-1} : \left|\hatberr{g,\pi^k,t} \right|\le \zetaelimin \right\}.$$
    \ENDIF
    \ENDFOR
     \end{algorithmic}	
    \end{routine}

\subsection{Analysis}
\tiancheng{Remark that we require weaker condition.}
We begin with the guarantee for the inner loop. This is just an application of the results in \cite{jin2021bellman}.
\begin{lemma}[Theorem 17 in \cite{jin2021bellman}]
    \label{lem:inner-olive}
    Given parameter $\epsilon$, there exists absolute constant $c$ such that if we choose 
    $$\zetaactin=\frac{2\epsilon}{H},\ \zetaelimin=\frac{\epsilon}{2H\sqrt{d_{\dagger}}},\ \nactin=\frac{H^2 \iota}{\epsilon^2},\text{ and } \nelimin=\frac{H^2d_{\dagger}\log(\Ncal_\Fcal(\zetaelimin/8)) \cdot \iota}{\epsilon^2}$$
     where   $\iota=c\log(Hd_{\dagger}/\delta\epsilon)$, 
     then with probability at least $1-\delta$, \olivebr (Routine~\ref{alg:olivemg-routine}) will output an $\Ocal(\epsilon)$-optimal policy using within  $\kin = \Ocal(H^3d_{\dagger}^2\log[\Ncal_\Fcal(\zetaelimin/8)] \cdot \iota/{\epsilon^2})$ episodes.   
\end{lemma}

\begin{remark}
    We need two assumptions to make the above guarantee hold:
    \begin{enumerate}
        \item Define the function class $\Fcal^{\mu,\dagger} :=(I-\Tcal^{\mu,\dagger})\Fcal$, then 
        $\dedim(\Fcal^{\mu,\dagger},\Dcal_{\mu},\epsilon/H) \le d_{\dagger}$ for any $\mu$. 
        \item For any policy $\mu$, $Q^{\mu,\dagger} \in \Fcal$.
    \end{enumerate}
    \tiancheng{Also maybe we don't need to coever the whole $\Fcal$, but only $\mu^{T}\Fcal$.}
\end{remark}

Now we can state and prove the theoretical guarantee for the nested version.
\begin{theorem}[\olivemg]
    \label{thm:outer-olive}
    There exists absolute constant $c$ such that if we choose 
    $$\zetaactout=\frac{2\epsilon}{H},\ \zetaelimout=\frac{\epsilon}{2H\sqrt{d_{\star}}},\ \nactout=\frac{H^2 \iota}{\epsilon^2},\text{ and } \nelimout=\frac{H^2d_{\star}\log(\Ncal_\Fcal(\zetaelimout/8)) \cdot \iota}{\epsilon^2}$$
     and choosing the parameter of inner loop (Routine~\ref{alg:olivemg-routine}) using parameter $\epsilon$, where   $\iota=c\log(Hd_{\star}/\delta\epsilon)$, 
     then with probability at least $1-\delta$, \olivemg (Algorithm~\ref{alg:olivemg}) will output an $\Ocal(\epsilon)$-optimal policy using at most  $\kout = \Ocal(H^4d_{\star}(d_{\star}+d_{\dagger}^2)\log[\Ncal_\Fcal(\zetaelimout/8)] \cdot \iota/{\epsilon^2})$ episodes.   
\end{theorem}

\begin{remark}
    We need two assumptions to make the above guarantee hold:
    \begin{enumerate}
        \item $d_{\star}=\dedim((I-\Tcal^{\star,\star})\Fcal,\Dcal_{\nash,\dagger},\epsilon/H)$. 
        \item $Q^{\star,\star} \in \Fcal$.
    \end{enumerate}
\end{remark}

\begin{proof}[Proof of Theorem~\ref{thm:outer-olive}]
   By Lemma~\ref{lem:olive-concentration}, since  $Q^{\star,\star}$ is not eliminated, the set $\Bcal^{k}$ will not be empty with high probability. Therefore, if we can show \olivemg\ terminates within $K \le d_{\star} H+1$ phases, then with high probability the output policy is  $5\epsilon$-optimal because 
\begin{align*}
    V^{\star}_1(s_1) - V_1^{\mu^K,\dagger}(s_1)
    &\overset{\left( i \right)}{\le} V^*_1(s_1) - V_1^{\mu^K,\nu^K}(s_1)  + \Ocal(\epsilon)\\
    & \overset{\left( ii \right)}{\le} \nash(f_1^K(s_1,\cdot,\cdot)) - V_1^{\mu^K,\nu^K}(s_1)+ \Ocal(\epsilon)\\
    & \overset{\left( iii \right)}{\le} \sum_{h=1}^{H} \Ecal(f^{K},\pi^K,h)+ \epsilon
    \le \Ocal(\epsilon).
    \end{align*}
where$(i)$ is by Lemma~\ref{lem:inner-olive}, $(ii)$ is by optimism, and $(iii)$ is by error decomposition in Proposition~\ref{prop:routine}. 

In order to prove that \olivemg\ terminates within $d_{\star} H+1$ phases, it suffices to show that for each $h\in[H]$, we can activate the elimination procedure at the $h^{\rm th}$ step for at most  $d$ times.

For the sake of contradiction, assume that \olivemg\ does not terminate in $d_{\star}H+1$ phases. Within these $d_{\star}H+1$ phases, there exists some $h \in [H]$ for which the activation process has been activated for at least $d_{\star}+1$ times. Denote by $k_1<\cdots<k_{d_{\star}+1} \le d_{\star}H+1 $ the indices of the phases where the elimination is activated at  the $h^{\rm th}$  step. By the high-probability events, for all $i<j\le d_{\star}+1$, we have $|\Ecal(f^{k_j},\pi^{k_i},h)|<2\zetaelimout$ and for all $l\le d_{\star}+1$, we have $\Ecal(f^{k_l},\pi^{{k_l}},h)>\zeta_{\rm act}/2$. This means for all $l \le d_{\star}+1$, we have both
$\sqrt{\sum_{i=1}^{l-1} \big(\Ecal(f^{k_l},\pi^{{k_{i}}},h)\big)^2}< \sqrt{d_{\star}}\times 2\zetaelimout = \epsilon/H$ and 
$\Ecal(f^{k_l},\pi^{{k_l}},h)>\zeta_{\rm act}/2 =\epsilon/H$.
	Therefore, the roll-in distribution of $\pi^{k_1},\ldots,\pi^{k_{d_{\star}+1}}$ at step $h$ is an $\epsilon/H$-independent sequence of length $d_{\star}+1$, which contradicts with the definition of BE  dimension.
	So \olive\ should terminate within $d_{\star} H+1$ phases.
	
In sum, with probability at least $1-\delta$, 
\olivemg\ will terminate and output a $\Ocal(\epsilon)$-optimal policy using at most 
$$
(d_{\star}H+1)(\nactout +\nelimout+\Ocal(H^3d_{\dagger}^2\log[\Ncal_\Fcal(\zetaelimout)] \cdot \iota/{\epsilon^2})) \le \Ocal(
\frac{3cH^3d_{\star}(d_{\star}+d_{\dagger}^2)\log(\Ncal_\Fcal(\zetaelimout/8))\cdot \iota}{\epsilon^2})$$
 episodes.
    
\end{proof}

\begin{lemma}[Concentration lemma for \olivemg]
    \label{lem:olive-concentration}
    With probability at least $1-\delta$,
 the following events hold for the first $d_{\star}H+1$ phases
    \begin{enumerate}
        \item  If the elimination procedure is activated at the $h^{\rm th}$ step in the $k^{\rm th}$ phase, then  $\Ecal(f^k,\pi^{k},h)>\zetaactout/2$ and all $f\in\Fcal$ satisfying $|\Ecal(f,\pi^{k},h)|\ge2\zetaelimout$ get eliminated.
        \item  If the elimination procedure is not activated in the $k^{\rm th}$ phase, then, $\sum_{h=1}^{H}\Ecal(f^k,\pi^{k},h)<2H\zetaactout=4\epsilon$.
        \item $Q^{\star,\star}$ is not eliminated. 
    \end{enumerate}   
\end{lemma}

\begin{proof}
    The proof is similar to the argument in Appendix D.2 of \cite{jin2021bellman}. For completeness, we include the whole proof as follows. 
   
\paragraph{Concentration in the activation procedure}
Consider a fixed $(k,h)\in[d_{\star}H+1]\times[H]$ pair.
By Azuma-Hoefdding's inequality, with probability at least $1-\frac{\delta}{8H(d_{\star}H^2+1)}$, we have 
$$
| \hatberr{f^k, \pi^{k}, h}  - \berr{f^k, \pi^{k}, h}| \le \Ocal\paren{\sqrt{\frac{\iota}{\nactout}}} \le \frac{\epsilon}{2H}\le \zetaactout/4,
$$
where the second inequality follows from $\nactout=CH^2\iota/\epsilon^2$ with $C$ being chosen large enough.

Take a union bound for all $(k,h)\in[d_{\star}H+1]\times[H]$, we have with probability at least $1-{\delta}/4$, the following holds for all $(k,h)\in[d_{\star}H+1]\times[H]$
$$
| \hatberr{f^k, \pi^{k}, h}  - \berr{f^k, \pi^{k}, h}|\le\zetaactout/4.
$$
By \olivemg\, if the elimination procedure is not activated in the  $k^{\rm th}$ phase, we have\\
 $\sum_{h=1}^{H}\hat{\Ecal}(f^k,\pi^{k},h)\le H\zetaactout$. Combine it with the concentration argument we just proved,
$$
\sum_{h=1}^{H}{\Ecal}(f^k,\pi^{k},h)\le 
\sum_{h=1}^{H}\hat{\Ecal}(f^k,\pi^{k},h) + \frac{H\zetaactout}{4} <\frac{5H\zetaactout}{4}.
$$
On the other hand, if the elimination procedure is activated at the $h^{\rm th}$ step in the $k^{\rm th}$ phase, then  $\hat{\Ecal}(f^k,\pi^{k},h)>\zetaactout$. Again combine it with the concentration argument we just proved,
$$
{\Ecal}(f^k,\pi^{k},h)\ge \hat{\Ecal}(f^k,\pi^{k},h)-\frac{\zetaactout}{4} > \frac{3\zetaactout}{4}.
$$


\paragraph{Concentration in the elimination procedure}
Now, let us turn to the elimination procedure. 
First, let $\Zcal$ be an ${\zetaelimout}/{8}$-cover of $\Fcal$ with cardinality 
$\Ncal_\Fcal(\zetaelimout/8)$. 
With a little abuse of notation, for every $f\in\Fcal$, define $\fhat=\argmin_{g\in\Zcal}\max_{h\in[H]}\|f_h-g_h\|_\infty$.
By applying Azuma-Hoeffding's inequality to all $(k,g)\in[d_{\star}H+1]\times\Zcal$ and taking a union bound, we have with probability at least $1-{\delta}/4$, the following holds for all $(k,g)\in[d_{\star}H+1]\times\Zcal$
$$
| \hatberr{g, \pi^{k}, h_k}  - \berr{g, \pi^{k}, h_k}| \le \zetaelimout/4.
$$

Recall that Algorithm \olivemg\ eliminates all $f$ satisfying $|\hatberr{f, \pi^{k}, h_k}| > \zetaelimout$ when the elimination procedure is activated at the $h^{\rm th}_{k}$ step in the $k^{\rm th}$ phase. 
Therefore, if 
$|\Ecal(f,\pi^{k},h_k)|\ge2\zetaelimout$, 
$f$ will be eliminated because 
\begin{align*}
	|\hat{\Ecal}(f,\pi^{k},h_k)|
&\ge |\hat{\Ecal}(\fhat,\pi^{k},h_k)|- 2\times \frac{\zetaelimout}{8}\\
&\ge  | \berr{\fhat, \pi^{k}, h_k}|  -\frac{\zetaelimout}{2}\\
&\ge | \berr{f, \pi^{k}, h_k}|  -\frac{\zetaelimout}{2}- 2\times \frac{\zetaelimout}{8}
> \zetaelimout.
\end{align*}
Finally, note that $\Ecal(Q^{\star,\star},\pi,h)\equiv 0$ for any $\pi$ and $h$. As a result, it will never be eliminated within the first $d_{\star}H+1$ phases because we can similarly prove 
$$|\hat{\Ecal}(Q^{\star,\star},\pi^{k},h_k)| \le  | \berr{Q^{\star,\star}, \pi^{k}, h_k}|  +\frac{3\zetaelimout}{4} < \zetaelimout.$$

{\bf Wrapping up}: take a union bound for the activation and elimination procedure, and conclude that the three events, listed at the beginning of this section, hold for the the first $d_{\star}H+1$ phases
 with probability at least $1-\delta/2$.
\end{proof}

==> checklist.tex <==
\clearpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    Yes.
  \item Did you describe the limitations of your work?
    Yes.
  \item Did you discuss any potential negative societal impacts of your work?
    No, this paper is purely theoretical.
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    Yes.
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    Yes, they are presented in Section 2.1.
	\item Did you include complete proofs of all theoretical results?
    Yes, they are in the appendix.
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    N/A.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
  N/A.
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    N/A.
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    N/A.
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
  N/A.
  \item Did you mention the license of the assets?
  N/A.
  \item Did you include any new assets either in the supplemental material or as a URL?
  N/A.
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
  N/A.
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
  N/A.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
  N/A.
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
  N/A.
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
  N/A.
\end{enumerate}

\end{enumerate}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old.tex <==
\section{Old contents}

\subsection{Contents in the previous version}


\subsubsection{Type-I complexity}

Define
$$
\fmu_f(s) := \argmax_{x\in\Delta_\Acal}\left(\min_{b\in\Bcal} x\trans f(s,\cdot,b)\right)
$$
and
$$
\fres_{f,g}(s) : = \argmin_{b\in\Bcal}\left(\fmu_f(s)\trans g(s,\cdot,b)\right)
$$
Let $\fcop_{f,g}:=(\fmu_f,\fres_{f,g})$ denote the concatenation of $\fmu_f$ and $\fres_{f,g}$.

\begin{definition}[Q-Bellman rank]
The Bellman rank is the minimum integer $d$ so that there exists $\phi_h: \Fcal\times\Fcal \rightarrow\R^d$ and $\psi_h:\Fcal\times \Fcal\rightarrow\R^d$ for each $h\in[H]$, such that for any $f,f',g,g'\in\Fcal$, the average Bellman error
\begin{align*}
\E \left[ (g_h-\Tcal^{\fmu_{g'}}g_{h+1})(s_h,a_h,b_h)  \mid s_h,a_h,b_h \sim \fcop_{f,f'} \right]	
=\langle \phi_h(f,f'),\psi_h(g,g')\rangle,
\end{align*}
where $\|\phi_h(f,f')\|_2,\|\psi_h(g,g')\|_2\le\zeta$, and $\zeta$ is the normalization parameter.
\end{definition}



\begin{definition}[Nash Bellman residual]
The Nash Bellman residual of function class $\Fcal$ is defined as $(I-\Tcal^*)\Fcal=\{\Fcal_h-\Tcal^* \Fcal_{h+1}\}_{h=1}^H$ where 
$\Fcal_h-\Tcal^* \Fcal_{h+1}= \{f_h-\Tcal^* f_{h+1}:\ f\in\Fcal\}$.
\end{definition}



\begin{definition}[Nash-BestResponse Bellman residual]
The Nash-BestResponse Bellman residual of function class $\Fcal$ is defined as $(I-\Tcal^{*,\dagger})\Fcal=\{\Fcal_h-\Tcal^{*,\dagger}\Fcal_{h+1}\}_{h=1}^H$ where 
$\Fcal_h-\Tcal^{*,\dagger}\Fcal_{h+1}= \{f_h-\Tcal^{\mu} f_{h+1}:\ f\in\Fcal,\ \mu\in\Pi_{\Fcal}^{\nash}\}$.
\end{definition}







We introduce the following distributions.
\begin{enumerate}
	\item $\Dcal_{\dirac}:=\{\Dcal_{\dirac,h}\}_{h\in[H]}$, where $\Dcal_{\dirac,h} = \{\delta_{(s, a,b)}(\cdot) | s\in\cS, a \in \cA, b\in\Bcal\}$, i.e. the collections of probability measures that put measure $1$ on single state-action pairs.
	\item $\Dcal_{\mu}:=\{\Dcal_{\mu,h}\}_{h\in[H]}$, where $\Dcal_{\mu,h}$ denotes the collection of all probability measures over 
	$\Scal\times\Acal\times\Bcal$ at the $h^\text{th}$ step, which can be generated by executing some $\fcop_{f,g}$ with $f,g\in\Fcal$. 
\end{enumerate}


\begin{definition}[$\epsilon$-online BE dimension]
$d_{\rm ol}(\epsilon,\Fcal)= \dim_{\rm DE}((I-\Tcal^{*})\Fcal,\Dcal_{\dirac},\epsilon)$.
\end{definition}

\begin{definition}[$\epsilon$-selfplay BE dimension]
 $d_{\rm sp}(\epsilon,\Fcal)= \min_{\Dcal\in\{\Dcal_\Delta,\Dcal_\mu\}} \dim_{\rm DE}((I-\Tcal^{*,\dagger})\Fcal,\Dcal,\epsilon)$.
\end{definition}

\subsubsection{Type-II complexity}

We redefine the following distributions for the type-II setting.

\begin{enumerate}
	\item $\Dcal_{\dirac}:=\{\Dcal_{\dirac,h}\}_{h\in[H]}$, where $\Dcal_{\dirac,h} = \{\delta_{s}(\cdot) | s\in\cS\}$, i.e. the collections of probability measures that put measure $1$ on single state-action pairs.
	\item $\Dcal_{\mu}:=\{\Dcal_{\mu,h}\}_{h\in[H]}$, where $\Dcal_{\mu,h}$ denotes the collection of all probability measures over 
	$\Scal$ at the $h^\text{th}$ step, which can be generated by executing some $\fcop_{f,g}$ with $f,g\in\Fcal$. 
\end{enumerate}

\begin{definition}[V-Bellman rank]
The Bellman rank is the minimum integer $d$ so that there exists $\phi_h: \Fcal^2 \rightarrow\R^d$ and $\psi_h:\Fcal^3\rightarrow\R^d$ for each $h\in[H]$, such that for any $f,f',g,g',\tilde g \in\Fcal$, the average Bellman error
\begin{align*}
\E \left[ g_h-\Tcal^{\fmu_{g'}}g_{h+1})(s_h,a_h,b_h)  \mid s_h \sim \fcop_{f,f'}, \ a_h,b_h\sim \fcop_{g',\tilde g}\right]	
=\langle \phi_h(f,f'),\psi_h(g,g',\tilde g)\rangle,
\end{align*}
where $\|\phi_h(f,f')\|_2,\|\psi_h(g,g',\tilde g)\|_2\le\zeta$, and $\zeta$ is the normalization parameter.
\end{definition}


\qinghua{We don't have the online version of type-II BE-dimension because $\nu^k$ is picked by the adversary.}


Denote function $v_{g,g',\tilde g,h}:\Scal\rightarrow\R$ such that for all $s\in\Scal$
$$v_{g,g',\tilde g,h}(s)=\E \left[ g_h-\Tcal^{\fmu_{g'}}g_{h+1})(s_h,a_h,b_h)  \mid s_h=s, \ a_h,b_h\sim \fcop_{g',\tilde g}(s)\right].$$
Let function class $\Vcal_h = \{v_{g,g',\tilde g,h}:  \ g,g',\tilde g \in \Fcal\}$.
Denote $\Vcal=\{\Vcal_h\}_{h\in[H]}$.
\begin{definition}[$\epsilon$-selfplay BE dimension]
 $d_{\rm sp, II}(\epsilon,\Fcal)= \min_{\Dcal\in\{\Dcal_\Delta,\Dcal_\mu\}} \dim_{\rm DE}(\Vcal,\Dcal,\epsilon)$.
\end{definition}











\subsection{Linear Quadratic Dynamics Games}
%\cite{pachter2010discrete,bu2019global} State transition is 
%$$
%s_{h+1}=Aa_h+Bb_h+Cs_h+w_h,
%$$
%where $w_h$ is a Gaussian noise term and reward of the max-player is 
%$$
%r\left( s,a,b \right) =a^TPa+b^TQb+s^TRs.
%$$
%which cannot be modeled by linear Markov Games \citep{xie2020learning} since the reward is not linear.

%\tiancheng{the most efficient way may be prove it has low Bellman rank but first we need to nail down what Bellman rank we really need.}
\begin{definition}[Linear Quadratic Dynamics Games \citep{pachter2010discrete,bu2019global} ]
	We say a MG is a finite-horizon discrete-time Linear Quadratic Dynamics Game (LQDG) if there exists 
	$A\in \R^{d\times d}$, $B_a\in\R^{d\times K_a}$, $B_b\in\R^{d\times K_b}$,  $Q\in\R^{d \times d}$, $P_a\in\R^{K_a \times K_a}$ and $P_b\in\R^{K_b \times K_b}$ such that
	for $h\in[H]$
	\begin{equation}
		\begin{aligned}
	&		s_{h+1} = A s_h + B_a a_h + B_b b_h + w_h, \\
	&       r(s_h,a_h,b_h) = s_h\trans Q  s_h -  a_h\trans P_a  a_h + b_h\trans P_b  b_h,
		\end{aligned}
	\end{equation}
where $\{w_h\}_{h=1}^H$ are zero-centered i.i.d. noise with $\E[w_h w_h\trans]= \Sigma$.
\end{definition}

\begin{lemma}
Suppose $\Mcal$ is a Linear Quadratic Dynamics Game.
	Consider $\Fcal=\Fcal_1 \times \Fcal_2 \times \cdots\times\Fcal_H$ with each $\Fcal_h$ defined as
	\begin{align*}
	\bigg\{ & s\trans M_s s - a\trans M_a a  + b\trans M_b b + s\trans M_{sa} a+ s\trans M_{sb} b
	+  a\trans M_{ab} b
	+\lambda: \\
&	M_s\in\R^{d \times d},\ M_a\in\R^{K_a \times K_a},\ M_b\in\R^{K_b \times K_b}, \ M_{sa}\in\R^{d \times K_a},\\
& M_{sb}\in\R^{d \times K_b}, \ M_{ab}\in\R^{K_a \times K_b},\ \lambda\in\R, \  
  M_a,M_b \succ 0\\
  & \mbox{and all matrices and scalar have Frobenius norm no larger than $\zeta$} 
  \bigg\}
%	 \ C_s\in\R^{d \times d},\ C_a\in\R^{d \times K_a},\ C_b\in\R^{d \times K_b} 
	\end{align*}
%	\ M_{s}\in\R^{d \times d}, \ M_{a}\in\R^{K_a \times K_a},\ M_{ab}\in\R^{K_a \times K_b},\ M_{b}\in\R^{K_b \times K_b}
Then $\Mcal$ and $\Fcal$ have Bellman rank at most $\Ocal(d^2+K_a^2+K_b^2)$.
\end{lemma}
%\qinghua{Its type-II Bellman rank is $\Ocal(d^2)$.}
\begin{remark}
	We comment that under certain necessary and sufficient conditions (c.f. Theorem 2.1 in \cite{pachter2010discrete}), a unique Nash equilibrium (Nash policy) is guaranteed to exist for $\Mcal$ and its corresponding action-value function belongs to $\Fcal$.
\end{remark}

\begin{proof}
	First recalling the definition of Bellman rank, we want to show there exist $\phi$ and $\psi$ such that the following decomposition holds for all $f,f',g,g'\in\Fcal$
	\begin{equation*}
\E_{\fcop_{f,f'}} [ g_h(s_h,a_h,b_h) - r_h(s_h,a_h,b_h) - \min_{b'} g_{h+1}(s_{h+1},\fmu_{g'}(s_{h+1}),b')]	=\langle \phi_h(f,f'),\psi_h(g,g')\rangle.
\end{equation*}

For notion simplicity, we define 
$$
v(s,a,b)=
{\rm Vec}\left(
\left(\begin{matrix}
	s\\
	a\\
	b\\
	1
\end{matrix}\right)
\left(s\trans,a\trans,b\trans,1\right)
\right)
$$
which is a $(d+K_a+K_b+1)^2$-dimensional feature vector. 
Note that $g_h(s,a,b) - r_h(s,a,b)$ is a linear function of 
$v(s,a,b)$ so there exists $\theta^g_h \in \R^{(d+K_a+K_b+1)^2}$ such that 
$$
g_h(s,a,b) - r_h(s,a,b) 
= \langle v(s,a,b), \theta_h^g\rangle.
$$
Therefore, 
\begin{equation*}
\E_{\fcop_{f,f'}} [ g_h(s_h,a_h,b_h) - r_h(s_h,a_h,b_h)]	=\langle \E_{\fcop_{f,f'}}[v(s_h,a_h,b_h)] ,\theta_h^g\rangle.
\end{equation*}

It remains to decompose $\E_{\fcop_{f,f'}}[\min_{b'} g_{h+1}(s_{h+1},\fmu_{g'}(s_{h+1}),b')]$.
By using the definition of $\Fcal$ and $\fmu_{g'}$, we have  $\fmu_{g'}$ is a linear policy, i.e., for all $h$, there exist $\Pi^{g'}_{h}\in\R^{d\times K_a}$ such that 
$$
\fmu_{g'}(s_{h}) = \Pi^{g'}_{h} s_h.
$$
As a result, one can easily verify by basic algebraic calculation that $\min_{b'} g_{h}(s,\fmu_{g'}(s),b')$ admits the following concise form
$$
\min_{b'} g_{h}(s,\fmu_{g'}(s),b')]
= s\trans O^{g,g'}_{h}s + o^{g,g'}_h
\quad \mbox{for all } s,
$$
where $O^{g,g'}_{h}\in\R^{d\times d}$ and $o^{g,g'}_{h}\in\R$ are determined by $g_{h}$ and $g'_h$. As a result, we obtain 
\begin{align*}
	\E_{\fcop_{f,f'}}[\min_{b'} g_{h+1}(s_{h+1},\fmu_{g'}(s_{h+1}),b')] = \langle \E_{\fcop_{f,f'}}[ s_{h+1} s_{h+1}\trans ],O^{g,g'}_{h+1} \rangle + o^{g,g'}_{h+1},
\end{align*}
which concludes the entire proof.
\end{proof}


\subsection{Linear MGs}
\begin{definition}[linear MGs]
We say an MG is linear of dimension $d$ if for each $h\in[H]$, there exist feature mappings $\phi_h: \Scal\times\Acal\times\Bcal\rightarrow\R^d$, $\psi_h: \Scal\rightarrow\R^d$ and vector $\theta_h^r\in\R^d$
such that $\Pr_h(s'\mid s,a,b)=\phi_h(s,a,b)\trans\psi_h(s')$ and $r_h(s,a,b)=\phi_h(s,a,b)\trans\theta_h^r$. 
\end{definition}


\begin{lemma}\label{lem:linear-Bellman}
	Suppose MGs $\Mcal$ is $d$-dimensional linear.	Define $\theta:=(\theta_1,\ldots,\theta_H)\in\R^{d\times H}$, and $f_{\theta,h}(s,a,b):=\phi_h(s,a,b)\trans\theta_h$ for all $(s,a,b)\in\Scal\times\Acal\times\Bcal$ and $h\in[H]$. 
	Then $\Mcal$ and $\Fcal:=\{f_\theta=(f_{\theta,1},\ldots,f_{\theta,H},0):\ \theta\in \R^{d\times H}\}$ have type-I Bellman rank at most $d$.
\end{lemma}
\begin{proof}
The proof follows directly from the definitions of linear MGs and Bellman rank.


Consider arbitrary $\theta,\theta'\in\R^{d\times H}$ and $h\in[H]$. 
Let $\pi$ be an arbitrary policy. We have
	\begin{equation}
		\begin{aligned}
			&\E_{\pi} [ f_{\theta,h}(s_h,a_h,b_h) - r_h(s_h,a_h,b_h) - \min_{b'} f_{\theta,h+1}(s_{h+1},\fmu_{f_{\theta',h+1}}(s_{h+1}),b')]\\
			= &\left\langle \E_\pi[\phi_h(s_h,a_h,b_h)]\ ,\ \theta_h-\theta_h^r - \sum_{s_{h+1}\in\Scal}
			\psi_{h}(s_{h+1})\min_{b'} f_{\theta,h+1}(s_{h+1},\fmu_{f_{\theta',h+1}}(s_{h+1}),b')
			\right\rangle
		\end{aligned}
	\end{equation}
We conclude the proof by noticing that the LHS of the inner product only depends on $(\pi,h)$ and the RHS is fully determined by $(f_\theta,f_{\theta'},h)$.
\end{proof}


\qinghua{linear kernel MDPs}


\subsection{Reactive POMGs}
%\qinghua{In order to define reactive POMGs, we have to define type-II Bellman rank.}
\begin{definition}[Reactive POMGs]
In reactive partially observable Markov games, the optimal action-value function $Q^*$ only depends on the latest observation and action, i.e., for all $h$, there exists $f^*_h: \Ocal\times \Acal\times\Bcal \rightarrow [0,1]$ such that for all $\tau_h = [o_1,a_1,b_1,\ldots,o_{h-1},a_{h-1},b_{h-1},o_h]$
$$
Q_h^*(\tau_h,a,b)
 = f_h^*(o_h,a,b)\  \mbox{ for all } (a,b)\in\Acal\times\Bcal.
$$
Moreover, any memoryless policy $\mu: \Ocal\rightarrow \Acal$ has at least one best-response policy  $\nu$ that is also memoryless and their action-value function $Q^{\mu,\nu}$ only depends on the latest observation and action, i.e., for all $h$, there exists $f^{\mu,\nu}_h: \Ocal\times \Acal\times\Bcal \rightarrow [0,1]$ such that for all $\tau_h = [o_1,a_1,b_1,\ldots,o_{h-1},a_{h-1},$
$b_{h-1},o_h]$
$$
Q_h^{\mu,\nu}(\tau_h,a,b)
 = f_h^{\mu,\nu}(o_h,a,b)\  \mbox{ for all } (a,b)\in\Acal\times\Bcal.
$$ 
\end{definition}

\begin{remark}
	A special case of reactive POMGs is block MGs
\end{remark}

\begin{lemma}
Any $\Fcal\subset (\Ocal\times\Acal\times\Bcal\rightarrow \R)$ and reactive MGs have type-II Bellman rank at most $|\Scal|$.
\end{lemma}
\begin{proof}
	The proof is exactly the same as that of proving reactive POMDPs have Bellman rank at most $|\Scal|$. 

To begin with, since any function in $\Fcal$ is memoryless, we have that $\fcop_{f,f'}$ is a function from $\Ocal$ to $\Delta_\Acal\times\Bcal$ for any $f,f'\in\Fcal$.
	
For any $h\in[H]$ and $f,f',g,g',\tilde g \in\Fcal$, 
\begin{align*}
 & \E \left[ (g_h-\Tcal^{\fmu_{g'},\dagger}g_{h+1})(\tau_h,a_h,b_h)  \mid \tau_h \sim \fcop_{f,f'}, \ a_h,b_h\sim \fcop_{g',\tilde g}\right]	\\
= & \E \Big[ g_h(o_h,a_h,b_h)-
r_h(o_h,a_h,b_h) - \min_{b}g_{h+1}(o_{h+1},\fmu_{g'}(o_{h+1}),b)   \mid s_h \sim \fcop_{f,f'},\\
&  o_h\sim\mathcal{O}_h(\cdot\mid s_h), \  (a_h,b_h)\sim \fcop_{g',\tilde g}(o_h),\ s_{h+1}\sim\mathbb{T}_h(\cdot\mid s_h,a_h,b_h),\ o_{h+1}\sim\mathcal{O}_h(\cdot\mid s_{h+1})\Big]\\
= & \sum_{s\in\Scal} \Pr^{\fcop_{f,f'}}(s_h=s) \cdot \E \Big[ g_h(o_h,a_h,b_h)-
r_h(o_h,a_h,b_h) - \min_{b}g_{h+1}(o_{h+1},\fmu_{g'}(o_{h+1}),b) \\
&  \mid o_h\sim\mathcal{O}_h(\cdot\mid s), \  (a_h,b_h)\sim \fcop_{g',\tilde g}(o_h),\ s_{h+1}\sim\mathbb{T}_h(\cdot\mid s,a_h,b_h),\ o_{h+1}\sim\mathcal{O}_h(\cdot\mid s_{h+1})\Big].
\end{align*}
Note the probability term only depends on $f,f'$ while 
the expectation term only depends on $g,g',\tilde g$, which concludes the proof.
\end{proof}




\subsection{Feature selection in linear MGs}

\paragraph{Problem formulation \citep{agarwal2020flambe}}
Let $\Mcal$ be a $d$-dimensional linear MG with respect to feature mapping $\phi^*$ and $\psi^*$ as well as reward parameter $\theta^r$.
Let $\Phi$ be  a feature class consisting of feature mappings  from $\Scal\times\Acal\times\Bcal\times[H]$ to $\R^d$, which satisfies $\phi^*\in\Phi$.
Give a pair of $\theta=(\theta_1,\ldots,\theta_H)\in\R^{d\times H}$ and $\phi\in\Phi$, we can naturally define an action-value function candiate $f^{\phi,\theta}=\{f^{\phi,\theta}_h\}_{h=1}^H$ such that  $f^{\phi,\theta}_h(s,a,b):=\phi_h(s,a,b)\trans\theta_h$ for all $(s,a,b)\in\Scal\times\Acal\times\Bcal$ and $h\in[H]$. 
Let $\Fcal^{\Phi} = \{ f^{\phi,\theta}:\ \theta\in\R^d,\ \phi\in\Phi\}$. Being provided with $\Fcal^\Phi$, the goal of feature selection is to learn an approximate Nash policy by interacting with $\Mcal$.  

 

\begin{lemma}\label{lem:linear-Bellman}
Any $d$-dimensional linear MG $\Mcal$ and function class $\Fcal$ have type-II Bellman rank at most $d$.
\end{lemma}
\begin{proof}
Suppose MG $\Mcal$ is $d$-dimensional linear with respect to feature mapping $\phi$ and $\psi$ as well as reward parameter $\theta^r$. Then for any $f,f',g,g',\tilde g \in\Fcal$,
\begin{align*}
&\E \left[ (g_h-\Tcal^{\fmu_{g'},\dagger}g_{h+1})(s_h,a_h,b_h)  \mid s_h \sim \fcop_{f,f'}, \ a_h,b_h\sim \fcop_{g',\tilde g}\right]	\\
= &\sum_{z\in\Scal\times\Acal\times\Bcal} \sum_{s} \Pr^\fcop_{f,f'}[(s_{h-1},a_{h-1},b_{h-1})=z] \times 
\Pr[s_{h}=s\mid (s_{h-1},a_{h-1},b_{h-1})=z]   \\
&\quad \quad \times\E \left[ (g_h-\Tcal^{\fmu_{g'},\dagger}g_{h+1})(s_h,a_h,b_h)  \mid s_h=s, \ a_h,b_h\sim \fcop_{g',\tilde g}(s)\right]	\\
= &\sum_{z\in\Scal\times\Acal\times\Bcal} \sum_{s\in\Scal} \Pr^\fcop_{f,f'}[(s_{h-1},a_{h-1},b_{h-1})=z] \times 
 \langle \phi_{h-1}(z),\psi_{h-1}(s)\rangle \\
&\quad \quad \times\E \left[ (g_h-\Tcal^{\fmu_{g'},\dagger}g_{h+1})(s_h,a_h,b_h)  \mid s_h=s, \ a_h,b_h\sim \fcop_{g',\tilde g}(s)\right]\\
= & \Big\langle \sum_{z\in\Scal\times\Acal\times\Bcal}  \Pr^\fcop_{f,f'}[(s_{h-1},a_{h-1},b_{h-1})=z] \times  \phi_{h-1}(z),\\
 & \quad\quad 
\sum_{s\in\Scal} \E \left[ (g_h-\Tcal^{\fmu_{g'},\dagger}g_{h+1})(s_h,a_h,b_h)  \mid s_h=s, \ a_h,b_h\sim \fcop_{g',\tilde g}(s)\right]\times \psi_{h-1}(s) \Big\rangle.
\end{align*}
We conclude the proof by noticing that the left part of the inner product only depends on $f,f'$ while the right part only depends on $g,g',\tilde g$.
\end{proof}
Since the result above holds for any function class $\Fcal$, the feature selection  problem for linear MGs shall have type-II Bellman rank at most $d$.




==> one_side.tex <==
\section{Why single side algorithm?}
The algorithmic solution proposed for tabular MG \cite{bai2020provable} and linear MG \cite{xie2020learning} can be seen as special cases of solving the following sub-problem: in each step $k$, given the confidence set of possible functions $f \in \Bcal^k$, find function pair $(f^k,g^k)$ and policy pair $(\mu^k.\nu^k)$ s.t. 
\begin{equation}
    \label{equ:sub-problem}
    \left< f^k,\mu ^k\times \nu ^k \right> \ge \underset{f\in \mathcal{B}^k,\mu}{\max}\left< f,\mu \times \nu ^k \right>, \,\,\,\,
    \left< g^k,\mu ^k\times \nu ^k \right> \le \underset{g\in \mathcal{B}^k,\nu}{\min}\left< g,\mu ^k\times \nu \right> .    
\end{equation}



Here we omit the dependence on $h$ by considering a single-horizon special case. This is similar to contextual bandit, but a game version.

Once the above sub-problem can be solved, using the fact that the true value function $f^{\star}$ is contained in $\Bcal^k$, we can bound the duality gap by 
$$
V^{\dagger ,\nu ^k}-V^{\mu ^k,\dagger}=\left< f^{\star},\left( \nu ^k \right) ^{\dagger}\times \nu ^k \right> -\left< f^{\star},\mu ^k\times \left( \mu ^k \right) ^{\dagger} \right> \le \left< f^k-g^k,\mu ^k\times \nu ^k \right> 
$$
and the standard arguemnt can be used to further bound this term by pigeon-hole argument.

Then a natural question is: how can we solve this sub-problem? A helpful condition is pointwise maximum/minimum completeness, which indeed holds for tabular and linear MG \cite{bai2020provable,xie2020learning}. For the max version, this means the pointwise upper bound defined by $\overline{f}^k\left( s,a,b \right) :=\underset{f\in \mathcal{B}^k}{\max}f\left( s,a,b \right)$ satistisfies $\overline{f}^k \in \Bcal^k$ (and of course $\overline{f}^k \in \Fcal$). The min version is similar.

Under this condition, the function pair $(\up{f}^k,\low{f}^k)$ is clearly the maximizer/minimizer and the sub-problem reduces to 
$$
\left< f^k,\mu ^k\times \nu ^k \right> \ge \underset{\mu}{\max}, \,\,\,\,   \left< f^k,\mu ^k\times \nu ^k \right> \le \underset{\nu}{\min}\left< f^k,\mu ^k\times \nu \right> ,
$$
which is just the Nash equilibrium.

\tiancheng{do we need to elaboarate on why these conditions hold for tabular and linear cases? This can be a little bit long since we need to introduce the notions for both.}

However, the pointwise maximum/minimum completeness may not hold in general. Even worse, no solution may exist for the sub-problem ~\eqref{equ:sub-problem}, as we will see below by a concrete example. In that case, the existing techniques fail and it's not clear how to bound the two-sided duality gap. As a result, the general function approximation problem is significantly harder than the special cases mentioned before.

Now we describe the concrete example, with one states and three actions for both players. Then $f$ is essentially a $3 \times 3$ matrix and we will use $M$ to represent such matrices. The ground truth is  
$$
M^{\star}=\left( \begin{matrix}
	0&		1&		-1\\
	-1&		0&		1\\
	1&		-1&		0\\
\end{matrix} \right) 
$$
which actually describes the pay-off matrix for roxk-paper-scissors game. Now there are 6 other matrices in our confidence set $\Bcal$,
$$
M_1=\left( \begin{matrix}
	0&		1.1&		-1\\
	-1&		0&		1\\
	1&		-1&		0\\
\end{matrix} \right) ,\,\, M_2=\left( \begin{matrix}
	0&		1&		-1.1\\
	-1&		0&		1\\
	1&		-1&		0\\
\end{matrix} \right) ,\,\, M_3=\left( \begin{matrix}
	0&		1&		-1\\
	-1.1&		0&		1\\
	1&		-1&		0\\
\end{matrix} \right) 
$$
$$
M_4=\left( \begin{matrix}
	0&		1&		-1\\
	-1&		0&		1.1\\
	1&		-1&		0\\
\end{matrix} \right) ,\,\, M_5=\left( \begin{matrix}
	0&		1&		-1\\
	-1&		0&		1\\
	1.1&		-1&		0\\
\end{matrix} \right) ,\,\, M_6=\left( \begin{matrix}
	0&		1&		-1\\
	-1&		0&		1\\
	1&		-1.1&		0\\
\end{matrix} \right) 
$$

Now suppose we find matrix pair $(A,B)$ and policy pair $(\mu,\nu)$ which solves the above sub-problem ~\eqref{equ:sub-problem}. Whatever $\nu$ is, the max-player can choose some matrix $A$ where the best response is a singleton. To see this, consider two scenarios:
\begin{itemize}
    \item $\nu=(1/3,1/3,1/3)$. Then the max-player can choose $M_1$ and play $\mu=(1,0,0)$.
    \item $\nu\ne (1/3,1/3,1/3)$. Then the max-player can choose $M$ and exploit the unblanced play.
\end{itemize}

Similarly, $\nu$ must also be a singleton that is the best response of $\mu$ under some matrix $B$. Finally we can check this, i.e. singletons are best responses to each other, is impossible whatever $(A,B)$ are.
